Image Quality and the Reliability of Fabric-Density Measurement: Counting Threads from Smartphone Photos Through a Pick Glass

Thread density, the threads per inch along and across a woven fabric, is a basic specification that buyers check whenever fabric is sold. Without laboratory instruments, inspectors count it slowly, by eye, through a pick glass, a folding 10$\times$ magnifier with a one-inch window. A smartphone photo through that glass could make the check faster and leave a record. We judge such a photo by what it is used for, as in task-based image quality: it is good if the thread count from it is within $\pm$5% of the true count, a common tolerance in fabric specifications. We introduce PickGlass-TPI: 76 factory scenes of 44 fabric patches, each counted in an open annotation tool by a textile-trained annotator, whose counts are the reference. On it we benchmark frontier and open vision-language models, CNNs, counting specialists and a training-free spectral counter (PG-Lattice). No method agrees with the reference within the tolerance. The best methods are off by about a quarter: a small open model that we tuned only on synthetic images (Molmo2-4B, 25%) is level with the best frontier model, GPT-6.1-sol (27% when asked directly, 25% given four magnified close-ups of the window). Both err less than a non-expert annotator (37%), but only the tuned model also beats, on both error measures, a baseline that guesses each scene's density as the average of the others. PG-Lattice most often repeats its count within 5% across two photos of the same patch, but its misses, like GPT-6.1-sol's errors, are often a factor of two. Even the reference repeats a count across such re-shoots only to a median 9%, so one photo cannot yet be shown to meet $\pm$5%; the image quality that matters is reliability across re-shoots. Generic no-reference quality scores chosen before labeling do not rank PG-Lattice's error, and generative enhancement raises perceptual scores but does not reliably improve the count.

==> tables/main150_rows_refB.tex <==
Non-expert annotator & 37.3 [31, 44] & 24 & 34 & 4 \\
Leave-one-out mean & 33.2 [28, 40] & 8 & 20 & 1 \\
\midrule
Log-Gabor bank & 37.7 [32, 44] & 30 & 36 & 7 \\
\rowcolor{black!6}\ours (ours) & 34.8 [28, 41] & 28 & 39 & 6 \\
Combined (\ours + log-Gabor) & 34.4 [28, 41] & \textbf{33} & 41 & \textbf{8} \\
\ours, ruler crop$^{75/76}$ & 37.9 [31, 45] & 27 & 39 & 3 \\
Cascade (\ours/GPT) & 34.5 [28, 41] & 27 & 41 & 5 \\
\midrule
CNN, synthetic (zero-shot) & 39.3 [32, 48] & 10 & 19 & 1 \\
CNN, + pseudo-labels$^\ast$$^{48/76}$ & 30.7 [24, 39] & 19 & 34 & 3 \\
CNN, trained on non-expert$^\ddagger$ & 28.1 [23, 34] & 14 & 30 & 3 \\
CNN--VLM ensemble$^\ddagger$ & 25.4 [21, 31] & 12 & 32 & 2 \\
\midrule
\rowcolor{black!6}Molmo2-4B + LoRA (ours) & 25.2 [21, 31] & 14 & 29 & 1 \\
CountGD, cells $\to$ lattice$^\ddagger$ & 28.5 [23, 35] & 17 & 28 & 4 \\
\midrule
GPT-6.1-sol (P1) & 27.1 [22, 33] & 26 & 40 & \textbf{8} \\
GPT-6.1-sol, insets$^\S$ & 24.9 [20, 31] & 26 & \textbf{45} & 6 \\
Claude Fable 5.1 & 38.0 [33, 44] & 8 & 12 & 1 \\
Gemini 3.1 Pro & 35.9 [30, 42] & 9 & 17 & 0 \\
Gemini 3.8 Flash & 31.2 [27, 37] & 7 & 19 & 0 \\
Qwen3.8-Max-Prime$^{72/76}$ & 32.0 [27, 37] & 8 & 19 & 1 \\
Qwen3.8-27B (open) & 74.7 [72, 78] & 0 & 0 & 0 \\
Gemma-4-26B (open) & 56.7 [53, 60] & 1 & 2 & 0 \\


==> tables/quality76_main_rowsB.tex <==
None (clean) & 100 & 100 \\
JPEG, $q$=50 / 20 & 96 / 83 & 96 / \textbf{88} \\
Noise, $\sigma$=10 / 40 & \textbf{93} / 82 & 92 / \textbf{86} \\
Shadow, 25 / 50\% area & \textbf{96} / \textbf{95} & 95 / 93 \\
Glare, 5 / 30\% area & \textbf{88} / 59 & 82 / \textbf{63} \\
Defocus, $\sigma$=1 / 3 / 6\,u & 97 / 70 / 55 & 97 / \textbf{75} / \textbf{57} \\
Motion, 5 / 10 / 30\,u & 54 / 34 / 36 & \textbf{61} / \textbf{55} / \textbf{63} \\
Downscale, $\times$2 / 4 / 8 & 79 / 68 / 42 & \textbf{87} / \textbf{70} / \textbf{46} \\
Corners, 2 / 5 / 10\% side & \textbf{91} / \textbf{51} / \textbf{13} & 86 / 47 / 12 \\

